A Temporal Logic for Asynchronous Hyperproperties

Hyperproperties are properties of computational systems that require more than one trace to evaluate, e.g., many information-flow security and concurrency requirements. Where a trace property defines a set of traces, a hyperproperty defines a set of sets of traces. The temporal logics HyperLTL and HyperCTL* have been proposed to express hyperproperties. However, their semantics are synchronous in the sense that all traces proceed at the same speed and are evaluated at the same position. This precludes the use of these logics to analyze systems whose traces can proceed at different speeds and allow that different traces take stuttering steps independently. To solve this problem in this paper, we propose an asynchronous variant of HyperLTL. On the negative side, we show that the model-checking problem for this variant is undecidable. On the positive side, we identify a decidable fragment which covers a rich set of formulas with practical applications. We also propose two model-checking algorithms that reduce our problem to the HyperLTL model-checking problem in the synchronous semantics.

==> discussion.tex <==
\section{Discussion}
\label{sec:disc}


\paragraph*{Linearizability} requires that any history of execution of a 
concurrent data structure (i.e., sequence of invocation and response by different threads) matches 
some sequential order of invocations and responses~\cite{hw90}:
%
\[
\varphi_{\mathbf{LNZ}} = \forall \pi.\exists \pi'.\Etau.\G_{\tjvar}(\mathsf{history}_\pi \Iff 
\mathsf{history}_{\pi'})\]
%
where $\mathsf{history}$ denotes method invocations by the different
threads and the response observed, trace $\pi$ ranges over the
concurrent data structure and $\pi'$ ranges over its sequential
counterpart.

\cesartodo{I am not sure this is correct. What is in
	$\mathsf{hisory}$? If it is call events and return events, then the
	calls cannot be aligned with a trajectory because in the sequential
	exeuction it is always C1R1C2R2C3R3 but concurrent execution it could be
	C3C2C1R2R1R3.
}



\paragraph*{Goguen and Meseguer's noninterference (GMNI)} stipulates
that, for all traces, the low-observable output must not change when
all high inputs are removed:
% 
\[
\varphi_{\mathbf{GMNI}} \DefinedAs
\forall \pi. \exists \pi'. \Etau.
(\G \lambda_{\pi'}) \, \And \, \G(\lo_\pi \Iff \lo_{\pi'})
\]
%
where $\lambda_{\pi'}$ expresses that all of the high inputs in the
current state of $\pi'$ have dummy value $\lambda$, and denotes
low-observable output proposition.

\paragraph*{Generalized noninterference (GNI)} permits nondeterminism in 
the behavior, but stipulates that low-security outputs may not be 
altered by the injection of high-security inputs:
%
\[
\varphi_{\mathbf{GNI}} \DefinedAs \forall \pi. \forall \pi'. \exists \pi''.
\Etau. \G(hi_\pi \Iff hi_{\pi''}) \; \And\;  \G(lo_{\pi'} \Iff lo_{\pi''})
\]
%
The trace $\pi''$ is an interleaving of the high inputs trace $\pi$
and the low inputs and outputs of the trace $\pi'$, hence, the
existential trajectories.
%
Notice that we employ two independent trajectories, as the patterns of
occurrence of $\hi$ (in $\pi$ and $\pi''$) and $\lo$ (in $\pi'$ and
$\pi''$) do not have to be the same.
%
Other forms of noninterference such as Focardi and Gorrieri's {\em
	bisimulation nondeducibility on compositions (BNDC)}~\cite{fg00},
which requires that a system should appear the same to a low observer
no matter with what other system it is composed (i.e., run in
parallel) and {\em Boudol and Castellani's noininterference
	(BCNI)}~\cite{bc02} can be specified in the same way, although
different interleavings may be obtained by different mechanisms.
%
Such mechanisms such as such as parallel composition, event
synchronization, or nondeterminism through memory footprint in
concurrent programs are generally at semanitc model level and are
orthogonal to high-level policy requirements.
%
It is important to emphasize that our notion of trajectories which
allow stutter steps can elegantly abstract semantic model details in
defining noninterference.

%\todo{GNI is decidable (coloring algorithm)}

\paragraph*{Not never terminates} requires that for every initial state, there 
is some terminating trace, but not all traces must terminate:
%
\[
\varphi_{\mathbf{NNT}} \DefinedAs \forall \pi. \exists \pi'.\exists \pi''.
(\pi[0] = \pi'[0] = \pi''[0]) \; \Into \;
(\F \, \term_{\pi'} \; \And \; \G \neg \term_{\pi''})
\]

%\todo{This one is actually CTL, therefore decidable.}



==> figs/Makefile <==
IPETOIPE=/Applications/Ipe.app/Contents/MacOS/ipetoipe
IPELATEXDIR=latex/
IPESTYLES=styles/

FILES=	state \
	state2 \
	ex1 ex2 ex3 ex4 asynctraj1_new synctraj1_new synctraj_new ks_new

ALL=$(addsuffix .pdf, ${FILES})

all: ${ALL}

%.pdf: %.ipe
	${IPETOIPE} -pdf $<

clean:
	rm -f ${ALL}


==> figs/latex/definitions.tex <==
\newcommand{\Terms}{\mathcal{T}}


%
\newcommand{\Str}{\mathcal{S}} \newcommand{\StrDesc}{\Rightarrow}
\newcommand{\StrReaches}{\StrDesc^*} \newcommand{\Desc}{\mapsto}
\newcommand{\DirDesc}{\rightarrow}
%
\newcommand{\RecDesc}{\twoheadrightarrow}
\newcommand{\AnyDesc}{\rightsquigarrow}
\newcommand{\AlphaDesc}{\dasharrow}
\newcommand{\ALPHADesc}[1]{\stackrel{#1}\dasharrow}
\newcommand{\Reaches}{\AnyDesc^*}
\newcommand{\Class}[1]{\ensuremath{[#1]}}
\newcommand{\EqSite}[2]{#1\equiv_{\Reactors}#2}
\newcommand{\LiveP}{\textsc{Live-P}\xspace}
\newcommand{\SchemaP}{\textsc{Schema-P}\xspace}
\newcommand{\BadP}{\textsc{Bad-P}\xspace} \newcommand{\INVname}{\phi}
\newcommand{\INV}{\ensuremath{\INVname}\xspace}
%
\newcommand{\INVnext}[2]{\ensuremath{\INVname_{#1}^{({#2})}}}
\newcommand{\INVclause}[1]{\ensuremath{\INVname[#1]}}
\newcommand{\INVnextclause}[3]{\ensuremath{\INVname_{#1}^{({#2})}[#3]}}
\newcommand{\React}[1]{\text{react}(#1)} \newcommand{\bisim}{\approx}
\newcommand{\Await}{\mathbf{await}} \newcommand{\When}{\mathbf{when}}
\newcommand{\Do}{\mathbf{do}} \newcommand{\Dec}{\texttt{--}}
\newcommand{\Inc}{\texttt{++}} \newcommand{\Width}{6em}
\newcommand{\Type}[1]{\hspace{-0.2em}:\hspace{-0.2em}#1} %
\newcommand{\LHeight}{\textit{lh}} \newcommand{\Height}{\textit{h}}
\newcommand{\owise}{\text{otherwise}}
\newcommand{\EmptyP}{\textsc{Empty-P}\xspace}
\newcommand{\AdequateP}{\textsc{Adequate-P}\xspace}
\newcommand{\BasicP}{\textsc{Basic-P}\xspace}
\newcommand{\BasicPRec}{\textsc{BasicRec-P}\xspace}
\newcommand{\EfficientP}{\textsc{Efficient-P}\xspace}
\newcommand{\kEfficientP}{\ensuremath{k}\textsc{-Efficient-P}\xspace}
\newcommand{\jEfficientP}{\ensuremath{j}\textsc{-Efficient-P}\xspace}
\newcommand{\Proc}{\mathcal{P}}
\newcommand{\WaitOnConnection}{\emph{WaitOnConnection}\xspace}
\newcommand{\WaitOnReactor}{\emph{WaitOnReactor}\xspace}
\newcommand{\process}{task\xspace}
\newcommand{\emprocess}{\emph{task}\xspace}
\newcommand{\processes}{tasks\xspace}
\newcommand{\emprocesses}{\emph{tasks}\xspace}
\newcommand{\subprocess}{sub-task\xspace}
\newcommand{\emsubprocess}{\emph{sub-task}\xspace}
\newcommand{\subprocesses}{sub-tasks\xspace}
\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\AllocName}{\textit{alloc}}
\newcommand{\Alloc}[1]{\textit{alloc\textup{(}[#1]\textup{)}}}
\newcommand{\AllocBigger}[1]{\textit{alloc.bigger\textup{(}#1\textup{)}}}
\newcommand{\AllocInc}[1]{\textit{alloc.inc\textup{(}#1\textup{)}}}
\newcommand{\AllocDec}[1]{\textit{alloc.dec\textup{(}#1\textup{)}}}
\newcommand{\p}[1]{\ensuremath{a[#1]}}
%
\newcommand{\Pplus}[1]{\ensuremath{A[#1]}}
\newcommand{\pnext}[2]{\ensuremath{a'_{#1}[#2]}}
\newcommand{\Pplusnext}[2]{\ensuremath{A'_{#1}[#2]}} %
\newcommand{\En}[2]{\mathit{En}_{#1}(#2)} %
\newcommand{\In}[2]{\mathit{In}_{#1}(#2)} %
\newcommand{\Out}[2]{\mathit{Out}_{#1}(#2)} %
\newcommand{\Pres}[1]{\mathit{pres}({#1})}
\newcommand{\Log}[1]{\mathit{log}\;#1}
\newcommand{\EnNm}{\ensuremath{\mathit{En}}}
\newcommand{\EnName}{\EnNm\xspace} 
%
\newcommand{\InNm}{\ensuremath{\mathit{In}}}
\newcommand{\InName}{\InNm\xspace} 
%
\newcommand{\OutNm}{\ensuremath{\mathit{Out}}}
\newcommand{\OutName}{\OutNm\xspace}
%
\newcommand{\StateSpace}{\ensuremath{\mathcal{S}}}
\newcommand{\phiStates}{\ensuremath{\INV\text{-states}}\xspace}
\newcommand{\phiState}{\ensuremath{\INV\text{-state}}\xspace}
\newcommand{\AlgName}{\textsc{Minimal}}
\newcommand{\Alg}[2]{\ensuremath{\AlgName(#1,#2)}}

%

\newcommand{\LangInf}{\Lang_\text{inf}} %
\newcommand{\ArrowType}{\SelectTips{cm}{}} %



 \newcommand{\SetCategory}{\mathcal{S}\textit{et}}


\newcommand{\RLTL}{RLTL\xspace}
\newcommand{\LTL}{LTL\xspace}
\newcommand{\MuCalculus}{\ensuremath{\mu\text{-calculus}}}
%
\newcommand{\nuTL}{\ensuremath{\nu\text{TL}}}

\newcommand{\semInf}[1]{\Lang_\omega(#1)}
\renewcommand{\sem}[1]{\Lang(#1)}
\newcommand{\Aut}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\AutA}{\Aut{A}}

\newcommand{\Prop}{\textit{Prop}}


\newcommand{\PreL} [1]{\ensuremath{\!\!\phantom{.}^{-}#1}}
\newcommand{\PostL}[1]{\ensuremath{#1^{-}}}
\newcommand{\PreR} [1]{\ensuremath{\phantom{.}^{+}#1}}
\newcommand{\PostR}[1]{\ensuremath{#1^{+}}}
\newcommand{\NoMove}[1]{{\ensuremath{#1^{0}}}}
\newcommand{\BasicProp}{\Bool(\Prop)}
\newcommand{\BminusProp}{\PostL{\Bool}(\Prop)}
\newcommand{\Segment}[3]{(#1,#2,#3)}
\newcommand{\Inv}[1]{\ensuremath{#1^{-1}}}
%\newcommand{\Segment}[3]{#1[#2,#3]}
\newcommand{\Pointed}[2]{(#1,#2)}
%\newcommand{\Pointed}[2]{#1^{#2}}
\newcommand{\NotFirst}{\ensuremath{\mathit{notfirst}}}
\newcommand{\First}{\ensuremath{\mathit{first}}}

\newcommand{\modelsLTL}{\models_{\textsc{LTL}}}



==> figs/latex/figures/figures.tex <==
%\UseComputerModernTips

\newcommand{\ST}[1]{**[F-]{\texttt{#1}}}
\newcommand{\PROC}[1]{**[F-:<40pt>]{\textit{#1}}}
\newcommand{\EmbeddedAppsST}{
  \ST{\begin{tabular}{c}Embedded\\Application\\(C sources)\end{tabular}}}
\newcommand{\DirectST}{
  \PROC{\begin{tabular}{c}\phantom{A}\\\Direct\\\phantom{a} \end{tabular}}}
\newcommand{\InstrumentedSourcesST}{
  \ST{\begin{tabular}{c}Instrumented\\Annotated\\C sources\end{tabular}}}
\newcommand{\RuntimeManagerST}{
  \PROC{\begin{tabular}{c}\Direct\\Runtime\\Manager\end{tabular}}}
\newcommand{\CompileLinkST}{
  \PROC{\begin{tabular}{c}Compile\\Link\end{tabular}}}
\newcommand{\EmbeddedAppExecST}{
  \ST{\begin{tabular}{c}Embedded\\Application\\(executable)\end{tabular}}}




\newcommand{\FlowFig}{
  {\scriptsize
   \xymatrix@W=4.5em @H=4em @R=0em @C=3em {
     & & \RuntimeManagerST \ar[dr] & & \\
     \EmbeddedAppsST\ar[r] & \DirectST\ar[ur]\ar[dr] & & 
     \CompileLinkST \ar[r] & \EmbeddedAppExecST\\
     & & \InstrumentedSourcesST \ar[ur] & & \\
   }}
}
  
\newcommand{\Queue}[1]{**[F-]{\textrm{#1}}}
\newcommand{\Proc}[1]{**[F-:<50pt>]{\textit{#1}}}
%\newcommand{\Proc}[1]{*++[o][F-]{\textit{#1}}}

\newcommand{\AdhocFig}{
  {\scriptsize
   \xymatrix@W=4em @H=1.5em @R=1.3em @C=5em {
                              & \Proc{user}\ar[dl] & \Queue{user}\ar[l] &  \\
     \Queue{input}\ar[r] & \Proc{router}\ar[ur]\ar[r]\ar[dr] & \Queue{broadcast}\ar[dr] & \\
     \Proc{generator}\ar[u] & \Proc{sender}\ar[ur] & \Queue{output}\ar[l] & \Proc{delay}\ar[l]
  }
}}

==> figs/latex/macros.tex <==
\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother

% \newcommand{\mymid}{\mathbin{\mid}}
% \newcommand{\Power}[3]{{#2}\!\mymid\!{#1}\rangle\!\rangle{#3}}
% \newcommand{\WeakPower}[3]{{#2}\mymid\!{#1}\rangle{#3}} %warning: not dual power!!
% \newcommand{\PowerSub}[3]{{#2}\mymid{#1}\rangle\!\rangle{#3}}
% \newcommand{\WeakPowerSub}[3]{{#2}\mymid{#1}\rangle{#3}} %warning: not dual power!!

\newcommand{\Always}{\LTLsquare}
%\newcommand{\Always}{\mathbf{G}}
\newcommand{\Event}{\LTLdiamond}
\newcommand{\Eventually}{\Event}
\newcommand{\Next}{\LTLcircle}
\newcommand{\Prev}{\LTLcircleminus}
\newcommand{\Previously}{\Prev}
\newcommand{\PrevNoFirst}{\LTLcircletilde}
\newcommand{\Before}{\PrevNoFirst}
\newcommand{\HasAlwaysBeen}{\LTLsquareminus}
\newcommand{\SoFar}{\HasAlwaysBeen}
\newcommand{\Once}{\LTLdiamondminus}
\newcommand{\Since}{\mathbin{\mathcal{S}}}
\newcommand{\BackTo}{\mathbin{\mathcal{B}}}
\newcommand{\WeakPrev}{\LTLcircletilde}
\renewcommand{\Until}{\mathbin{\mathcal{U}}}
\newcommand{\WaitFor}{\mathbin{\mathcal{W}}}


%\newenvironment{proposition}{\theoremlike{Proposition}}{\par\medskip}

\newcommand{\val}[1]{\ensuremath{[\![ #1 ]\!]}}

\newcommand{\der}[1]{\ensuremath{\;\;{\mathop{{ %
            \longrightarrow}}\limits^{{#1}}}\!}\;\;} %

\newcommand{\Der}[1]{\ensuremath{\rightarrow_{#1}}} %
\newcommand{\notDer}[1]{\ensuremath{\not\rightarrow_{#1}}} %
%\newcommand{\notDer}[1]{\ensuremath{\;\;\not\rightarrow_{#1}\;\;}} %


\newcommand \tpl[1]{\langle #1 \rangle}


\newcommand{\LTL}{\textsf{LTL}\xspace}
\newcommand{\ForSpec}{\textsf{ForSpec}\xspace}

\newcommand{\SVA}{\textsf{SVA}\xspace}
\newcommand{\VLTL}{\textsf{VLTL}\xspace}
\newcommand{\RLTL}{\textsf{RLTL}\xspace}
%\newcommand{\RE}{\textsf{RE}\xspace}
\newcommand{\NVPA}{\textsf{NVPA}\xspace}
\newcommand{\VPA}{\textsf{VPA}\xspace}
\newcommand{\NFA}{\textsf{NFA}\xspace}
\newcommand{\VPL}{\textsf{VPL}\xspace}
\newcommand{\CARET}{\textsf{CaRet}\xspace}
\newcommand{\VPLs}{\textsf{VPL}s\xspace}
\newcommand{\VRL}{\textsf{VRL}\xspace}
\newcommand{\VRE}{\textsf{VRE}\xspace}
\newcommand{\EMSO}{\textsf{MSO$_{\mu}$}\xspace}
\newcommand{\MSO}{\textsf{MSO}\xspace}
\newcommand{\FO}{\textsf{FO}\xspace}
\newcommand{\EFO}{\textsf{FO}$_{\mu}$\xspace}
\newcommand{\XML}{\textsf{XML}\xspace}
%\newcommand{\ETL}{\textsf{ETL}\xspace}
\newcommand{\PDL}{\textsf{PDL}\xspace}
\newcommand{\AJA}{\textsf{AJA}\xspace}
\newcommand{\AJT}{\textsf{AJT}\xspace}
\newcommand{\SAJA}{\textsf{SAJA}\xspace}
\newcommand{\MAJA}{\textsf{MAJA}\xspace}
\newcommand{\AFA}{\textsf{AFA}\xspace}
\newcommand{\AVPA}{\textsf{AVPA}\xspace}
\newcommand{\PSL}{\textsf{PSL}\xspace}

\newcommand{\NWTL}{\textsf{NWTL}\xspace}
\newcommand{\NWTLPLUS}{\textsf{NWTL}$^{+}$\xspace}


\newcommand{\TWOEXPTIME}{\textsf{2-EXPTIME}\xspace}
\newcommand{\EXPTIME}{\textsf{EXPTIME}\xspace}
\newcommand{\PTIME}{\textsf{PTIME}\xspace}

\newcommand{\WM}{\ensuremath{\mathit{WM}}}
\newcommand{\MR}{\ensuremath{\mathit{MR}}}
\newcommand{\MC}{\ensuremath{\mathit{MC}}\xspace}
\newcommand{\SWM}{\ensuremath{\mathit{MWM}}\xspace}
\newcommand{\Pu}{\ensuremath{\mathcal{P}}}
\newcommand{\Lang}{\ensuremath{\mathcal{L}}}
\newcommand{\Au}{\ensuremath{\mathcal{A}}}
\newcommand{\Gam}{\ensuremath{\mathcal{G}}}
\newcommand{\Tu}{\ensuremath{\mathcal{T}}}
\newcommand{\Stratum}{\ensuremath{\mathcal{S}}}
\newcommand{\RejMain}{\ensuremath{\bot_\MainStates}}
\newcommand{\RejSec}{\ensuremath{\bot_\SecStates}}

%%%%
%%%% The following three macros are confusing with MainStates and SecStates
%%%%
\newcommand{\Msubst}{$M$-substitution\xspace} % M-substitution CHANGE FONT
\newcommand{\Mclosure}{$M$-closure\xspace}    %
\newcommand{\Sclosure}{$S$-closure\xspace}    %

\newcommand{\Region}{\ensuremath{\mathcal{R}}}

%\newcommand{\MainStates}{\ensuremath{\textit{M}}}
%\newcommand{\MainStates}{\ensuremath{M}}
\newcommand{\MainStates}{\ensuremath{\mathsf{M}}}
%\newcommand{\SecStates}{\ensuremath{\textit{S}}}
%\newcommand{\SecStates}{\ensuremath{S}}
\newcommand{\SecStates}{\ensuremath{\mathsf{S}}}
%\newcommand{\FamStratum}{\ensuremath{\mathfrak{F}}}
\newcommand{\FamStratum}{\ensuremath{\mathsf{F}}}
\newcommand{\Acc}{\ensuremath{\textit{Acc}}}
\newcommand{\Inf}{\ensuremath{\textit{Inf}}}
\newcommand{\SF}{\ensuremath{\textit{SF}}}
\newcommand{\Model}{\ensuremath{\textit{X}}}



\newcommand{\Stilde}{\widetilde{\Sigma}\xspace}
\newcommand{\Scall}{\Sigma_{\mathit{call}}}
\newcommand{\call}{{\mathit{call}}}
\newcommand{\ret}{{\mathit{ret}}}
\newcommand{\intA}{{\mathit{int}}}
\newcommand{\Sret}{\Sigma_{\mathit{ret}}}
\newcommand{\Sint}{\Sigma_{\mathit{int}}}

\newcommand{\Nat}{\mathbb{N}}



\newcommand{\SubstOp}[1]{\mathrel{\curvearrowleft_{#1}}}
\newcommand{\SubstBox}{\SubstOp{\Box}}
\newcommand{\MClos}[2]{#1^{\SubstOp{#2}}}
\newcommand{\LangClos}{\MClos{\Lang}{\Box}}
\newcommand{\SClos}[2]{{#1}^{\circlearrowleft_{#2}}}
\newcommand{\SClosure}[1]{\SClos{#1}{\Box}}
\newcommand{\LangSClos}{\SClos{\Lang}{\Box}}

\newcommand{\caller}{\mathsf{c}}
\newcommand{\down}{\mathsf{+}}
\newcommand{\abs}{\mathsf{a}}
\newcommand{\absExt}{\mathsf{ea}}
\newcommand{\PosBool}{\ensuremath{\mathcal{B}^{+}}}

%\newcommand{\dirUp}{\ensuremath{\uparrow}}
\newcommand{\dirUp}{\ensuremath{\leftarrow}}
%\newcommand{\dirDown}{\ensuremath{\downarrow}}
\newcommand{\dirDown}{\ensuremath{\rightarrow}}
%\newcommand{\dirUpAbs}{\ensuremath{\uparrow^{\abs}}}
\newcommand{\dirUpAbs}{\ensuremath{\curvearrowleft}}
%\newcommand{\dirDownAbs}{\ensuremath{\downarrow_{\abs}}}
\newcommand{\dirDownAbs}{\ensuremath{\curvearrowright}}
%\newcommand{\dirDownAbsExt}{\ensuremath{\downarrow_{\absExt}}}
%\newcommand{\dirDownAbsExt}{\ensuremath{\curvearrowright_{\mkern-15.2mu\raisebox{.30em}{$\phantom{.}_{\bullet}$}}}}
\newcommand{\dirDownAbsExt}{\ensuremath{\curvearrowright_{\mkern-8.5mu{\bullet}}}}
%\newcommand{\dirUpAbsExt}{\ensuremath{\uparrow^{\absExt}}}
%\newcommand{\dirUpAbsExt}{\ensuremath{\curvearrowleft_{\mkern-30.2mu\raisebox{.30em}{$\phantom{.}_{\bullet}$}}}}
\newcommand{\dirUpAbsExt}{\ensuremath{\phantom{.}_\bullet{\mkern-8.2mu\curvearrowleft}}}

\newcommand{\DIR}{\textit{DIR}}
\newcommand{\Trans}{\texttt{t}}
\newcommand{\Moves}{\textit{Moves}}
%\newcommand{\dir}{\textit{dir}}
\newcommand{\SUCC}{\mathsf{succ}}
\newcommand{\NULL}{\mathsf{\bot}}
\newcommand{\acc}{\textit{acc}}
\newcommand{\rej}{\textit{rej}}
\newcommand{\rank}{\textit{rank}}
\newcommand{\widt}{\textit{width}}

\newcommand{\DefinedAs}{\,\stackrel{\text{def}}{=}\,}

%\newcommand{\DefOR}{\ensuremath{\;\;\;\big|\;\;\;}}
\newcommand{\DefORmini}{\ensuremath{\;\big|\;}}

\newcommand{\details}[1]{}

%%%%%% Temporal Modalities %%%%%%%%%%%%%%

\newcommand{\true}{\ensuremath{\textup{\texttt{true}}}}
\newcommand{\false}{\ensuremath{\textup{\texttt{false}}}}
\newcommand{\Power}[3]{\mathrel{{#1}|{#2}\rrangle{#3}}}
\newcommand{\Norm}[1]{\ensuremath{\|{#1}\|}}
\newcommand{\WeakPower}[3]{\mathrel{{#1}|{#2}\rangle{#3}}}
\newcommand{\PastPower}[3]{\mathrel{{#1}\llangle{#2}|{#3}}}
\newcommand{\PastWeakPower}[3]{\mathrel{{#1}\langle{#2}|{#3}}}
%\newcommand{\Next}{\ensuremath{\bigcirc}}
\newcommand{\Seq}{\ensuremath{;}}
%\newcommand{\Previous}{\ensuremath{{\mathrlap{\bigcirc}\,\minus\,}}}
\newcommand{\Previous}{\Prev}
%\newcommand{\until}{{\sf U}}
\newcommand{\until}{\Until}
%\newcommand{\since}{{\sf S}}
\newcommand{\since}{\Since}
%\newcommand{\sometimes}{\lozenge}
%\newcommand{\always}{\square}
\newcommand{\always}{\Always}

\newcommand{\comp}[1]{\ensuremath{\overline{#1}}} % complement automaton
\newcommand{\dual}[1]{\ensuremath{\widetilde{#1}}} % dualization

\newcommand{\Outcm}{c\,b\,r}
\newcommand{\UOutcm}{\underline{\Outcm}}

\newenvironment{changemargin}[2]{%
  \begin{list}{}{%
    \setlength{\topsep}{0pt}%
    \setlength{\leftmargin}{#1}%
    %\setlength{\footnotewidth}{#1}%
    \setlength{\rightmargin}{#2}%
    \setlength{\textheight}{21cm}%
   \setlength{\topmargin}{0cm}
   \setlength{\listparindent}{\parindent}%
    \setlength{\itemindent}{\parindent}%
    \setlength{\parsep}{\parskip}%
  }
  \item[]}{\end{list}}


\newcommand{\push}{\textit{push}}
\newcommand{\Regions}{\ensuremath{\textit{REG}}}
\newcommand{\pop}{\textit{pop}}
%\newcommand{\pending}{\ensuremath{\texttt{pending}}}

\newcommand{\Bu}{\ensuremath{\textsf{B}}}
\newcommand{\Co}{\ensuremath{\textsf{C}}}

\newcommand{\alphaANY}{\ensuremath{\alpha_{\mathit{ONE}}}}

%%%% ATTENTION HERE: DON'T USE OLD DEFINITION IN FSTTCS CLASS iS treated as a section %%%%
\newcommand{\myparagraph}[1]{\paragraph{\textup{\textbf{#1}}}}
%\newcommand{\myparagraph}[1]{\noindent\textbf{#1}}

\newcommand{\myparagraphApp}[1]{\vspace{0.5em}\noindent\textup{\textbf{#1}}}

\newcommand{\qin}{\ensuremath{q_{\textit{in}}}}

==> figs/latex/macros/altba.tex <==
\newcommand{\var}{{\mathcal{X}}}
\newcommand{\posform}[1]{\mathcal{B}^+(#1)}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> figs/latex/macros/automata.tex <==
%\newcommand{\AutNode}[1]{*+[F-:<3pt>]{#1}}
\newcommand{\AutNode}[1]{*+[o][F-]{#1}}
\newcommand{\AutFinalNode}[1]{*+[o][F=]{#1}}

==> figs/latex/macros/colors.tex <==
\newcommand{\VLC}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\VRC}[1]{\textcolor{darkred}{#1}}
\newcommand{\emphC}[1]{\textcolor{red}{#1}}
\newcommand{\GR}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\RD}[1]{\textcolor{darkred}{#1}}
\newcommand{\BL}[1]{\textcolor{darkblue}{#1}}
\newcommand{\ORN}[1]{\textcolor{darkorange}{#1}}
\newcommand{\ColRE}[1]{\ORN{#1}}
\newcommand{\ColTL}[1]{\RD{#1}}
\newcommand{\ColAUT}[1]{\BL{#1}}
\newcommand{\ColL}[1]{\GR{#1}}

\newcommand{\Cr}{\ColRE{r}}
\newcommand{\Cs}{\ColRE{s}}
\newcommand{\Cx}{\ColTL{x}}
\newcommand{\Cy}{\ColTL{y}}
\newcommand{\Cz}{\ColTL{z}}
\newcommand{\spc}{\hspace{2em}}
\newcommand{\one}{\ColRE{\textit{one}}}
\newcommand{\mwm}{\ColRE{\textit{mwm}}}
\newcommand{\wm}{\ColRE{\textit{wm}}}
\newcommand{\mr}{\ColRE{\textit{mr}}}
\newcommand{\ttrue}{\ColTL{\texttt{true}}}
\newcommand{\Henceforth}{\ColTL{\textbf{G}}}
\newcommand{\ABS}{\ColRE{\textit{abs}}}
\newcommand{\CALLER}{\ColRE{\textit{caller}}}
\newcommand{\sumOne}{\ColRE{\textit{sum1}}}
\newcommand{\sumTwo}{\ColRE{\textit{sum2}}}
\newcommand{\Aut}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\AutA}{\Aut{A}}


==> figs/latex/macros/direct.tex <==
\newcommand{\Direct}{\textsc{Direct}\xspace}
\newcommand{\into}{\rightarrow}

%%%% FIGURE WITH 2 PROGRAMS
\begin{SaveVerbatim}[fontfamily=courier]{Thread-1}
1  void infa(void)  {
2    while (1) {
3      if (exp) {
4        mutex_lock(b);
5        mutex_lock(a);
6        // critical sect
7        mutex_unlock(a);
8        mutex_unlock(b);
9     } else {
10       mutex_lock(c);
11       mutex_lock(a);
12       // critical sect
13       mutex_unlock(a);
14       mutex_unlock(c);
15     }
16   }
17 }
\end{SaveVerbatim}

\begin{SaveVerbatim}[fontfamily=courier]{Thread-2}
21 void infb(void) {
22   while (1) {
23     mutex_lock(a);
24     mutex_lock(b);
25     // critical sect
26     mutex_unlock(b);
27     mutex_unlock(a);
28   }
29 }
\end{SaveVerbatim}

%%%%% TRACE OF DINING PHILOSPHERS
\newcommand{\DiningTrace}{
\begin{tabular}{|l||l|l|l|l|l|l|l|l|l|}
        \hline
$\textit{State}$ & $\textit{Thrd}$ & 
\multicolumn{5}{|c|}{\textit{Philosopher threads}} & \textit{Res} & \textit{Res} & $\textit{(c)alls/}$ \\
$\textit{no.}$ & $\textit{id}$ & $T_0$ & $T_1$ & $T_2$ & $T_3$ & $T_4$ & $\textit{values}$ & $\textit{held}$ & $\textit{(r)ets}$ \\
        \hline \hline
$1$  & $3$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 1)$ &  $(0, 0)$ & $(0,0,0,1,1)$ & $()$ & $c$ \\
\rowcolor[rgb]{0.90,0.99,0.90}$2$  & $3$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 1)$ &  $(0, 0)$ & $(0,0,0,0,1)$ & $(3)$ & $r$ \\
$3$  & $3$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 0)$ & $(0,0,0,0,1)$ & $(3)$ & $c$ \\
$4$  & $4$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 0)$ & $(0,0,0,0,1)$ & $()$ & $r$ \\
\rowcolor[rgb]{0.99,0.90,0.90}$5$  & $4$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 1)$ & $(0,0,0,0,1)$ & $()$ & $c$ \\
\rowcolor[rgb]{0.99,0.80,0.80}$6$  & $4$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 1)$ & $(0,0,0,0,0)$ & $(4)$ & $r$ \\
$\ldots$  & $\ldots$ &  &  &  &  &  & & & \\
$16$ & $4$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 2)$ & $(0,0,0,0,0)$ & $(4)$ & $r$ \\
\rowcolor[rgb]{0.90,0.70,0.70}$17$ & $4$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ & $(0,0,0,0,0)$ & $(4)$ & $c$ \\
        \hline
\end{tabular}
}



==> figs/latex/macros/enriched.tex <==
%%%%% %%%%% 1. for the enriched paper %%%%%
%\newcommand{\F}{\mathsf{F}} %\newcommand{\T}{\mathsf{T}}
%\newcommand{\F}{\mathbf{false}}
%\newcommand{\T}{\mathbf{true}}
%\newcommand{\true}{\T}
%\providecommand*{\Always}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Always}{\LTLsquare}
%\providecommand*{\Event}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Event}{\LTLdiamond}
%\providecommand*{\Next}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Next}{\LTLcircle}
%\newcommand{\Prev}{\LTLcircleminus}
%\newcommand{\PrevNoFirst}{\LTLcircletilde}
%\newcommand{\HasAlwaysBeen}{\LTLsquareminus}
%\providecommand*{\Once}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Once}{\LTLdiamondminus}
%\providecommand*{\Since}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Since}{\mathbin{\mathcal{S}}}
%\providecommand*{\BackTo}{} %Ale: to compile with cesar-llncs
%\renewcommand{\BackTo}{\mathbin{\mathcal{B}}}
%\newcommand{\WeakPrev}{\LTLcircletilde}


\newcommand{\ORsym}{{\scriptstyle{\pmb{+}}}}
\newcommand{\SEQsym}{{\scriptstyle{\cdot}}}
\newcommand{\ANDsym}{{\scriptstyle{\pmb{|}}}}
\newcommand{\STARsym}{*}
\newcommand{\EXPsym}{\widehat{\;\phantom{\cdot}\;}}
\newcommand{\POWsym}{\EXPsym}
\newcommand{\DPOWsym}{\_}
\newcommand{\NEGsym}{\overline{\;\phantom{\cdot}\;}}
%\newcommand{\INF}[1]{\overset{\infty}{#1}}
\newcommand{\INF}[1]{\widehat{#1}}
%\newcommand{\ORsymInf}{\INF{\ORsym}}
\newcommand{\ORsymInf}{\oplus}
%\newcommand{\ANDsymInf}{\INF{\ANDsym}}
\newcommand{\ANDsymInf}{\oslash}
%\newcommand{\SEQsymInf}{\INF{\SEQsym}} 
\newcommand{\SEQsymInf}{\odot} 
\newcommand{\OR}{\mathrel{+}}
\newcommand{\AND}{\mathrel{|}} 
\newcommand{\SEQ}{\mathrel{\cdot}}
%\newcommand{\ORInf}{\mathrel{\INF{\scriptstyle{+}}}}
\newcommand{\ORInf}{\mathrel{\oplus}}
%\newcommand{\ANDInf}{\mathrel{\INF{\scriptstyle{|}}}}
\newcommand{\ANDInf}{\mathrel{\oslash}}
%\newcommand{\SEQInf}{\mathrel{\INF{\scriptstyle{\cdot}}}}
\newcommand{\SEQInf}{\mathrel{\odot}}

\newcommand{\uSTAR}{^\STARsym} %unary star
\newcommand{\bSTAR}{\mathrel{\STARsym}} %unary star
\newcommand{\STAR}{\uSTAR} \newcommand{\CIRC}{\mathrel{\circ}}
%\newcommand{\EnrichedRE}{E$\omega${}RE\xspace}
\newcommand{\EnrichedRE}{\ensuremath{\textup{EnRE}}\xspace}
\newcommand{\EnRE}{\EnrichedRE}
\newcommand{\VeryEnrichedRE}{kE$\omega${}RE\xspace}
%\newcommand{\Vars}{\mathcal{V}}
\newcommand{\ElemRE}{\ensuremath{\textup{ElemRE}}\xspace}
%\newcommand{\Bool}{\mathcal{B}}
\newcommand{\wRE}[1]{\ensuremath{\omega\text{RE}(#1)}}
\newcommand{\finRE}[1]{\ensuremath{\text{RE}(#1)}}
\newcommand{\RE}{\textup{RE}\xspace} % regular expressions
\newcommand{\ERE}{\textup{ERE}\xspace} % Extended Regular Expressions RE(+,*,;,|,~,[w]) 
\newcommand{\SERE}{\textup{SERE}\xspace} %Semi-Extended Regular Expressions RE(+,*,;,|, ,[w])

\newcommand{\SigmaElem}{\Sigma_\text{elem}}
\newcommand{\SigmaEnriched}{\Sigma_\text{rich}}
\newcommand{\SigmaEnrichedInf}{\Sigma^{\omega}_\text{rich}}
\newcommand{\SigmaRegexp}{\Sigma_\text{regexp}}

\newcommand{\NBW}{NBW\xspace} % non-deterministic B\"uchi automata on words 
\newcommand{\DBW}{DBW\xspace} % deterministic B\"uchi automata on words 
\newcommand{\ABW}{ABW\xspace} % alternating B\"uchi automata on words 
\newcommand{\BABW}{BABW\xspace} %
\newcommand{\ETL}{\text{ETL}\xspace} % Extended Temporal Logic ETL
\newcommand{\ETLr}{\ensuremath{\text{ETL}_r}\xspace} % ETL (regular condition) 
\newcommand{\ETLl}{\ensuremath{\text{ETL}_l\xspace}} % ETL (loop condition) 
\newcommand{\ETLf}{\ensuremath{\text{ETL}_f\xspace}}
% ETL (finite condition)
\newcommand{\ETLa}{\ensuremath{\text{ETL}_a\xspace}} % ETL(alternating condition)
\newcommand{\ETLta}{\ensuremath{\text{ETL}_2a}\xspace} % ETL (two way alternating condition) 
\newcommand{\Release}{\mathbin{\mathcal{R}}}

\newcommand{\ALL}{\ensuremath{\mathbf{all}}\xspace}

%\newcommand{\Alphabet}{\Gamma}
\newcommand{\Alphabet}{\Sigma}

\newcommand{\Eqs}{\mathcal{E}}


\newcommand{\DefOR}{\ensuremath{\;\;\;\big|\;\;\;}}
\renewcommand{\SEQsym}{\ensuremath{;}}
\renewcommand{\SEQ}{\mathrel{\SEQsym}}

\newcommand{\REOR}{+}
\newcommand{\RESEQsym}{\ensuremath{;}}
\newcommand{\RESeq}{\mathrel{\RESEQsym}}
\newcommand{\REStar}{*}


==> figs/latex/macros/general.tex <==
\newcommand\Def[2][]{%                        % F"ur Definitionen 
  \def\temp{#1}%                              % die in den Index sollen
  \ifx\temp\empty%
    \def\temp{#2}%
  \fi%
%{\em\boldmath#2\unboldmath\index{\temp}}}
{\em#2\index{\temp}}}

\newcommand{\N}{\mathbb{N}}

\newcommand{\onlyWithComplement}[1]{}

%\newcommand{\pos}{\textit{pos}}
%\newcommand{\Pos}{\textit{Pos}}
\newcommand{\pos}{\omega}
\newcommand{\Pos}{\omega}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> figs/latex/macros/macros.tex <==
\input{macros/general}
\input{macros/enriched}
\input{macros/rules}
\input{macros/altba}
\input{macros/automata}
\input{macros/direct}
\input{macros/colors}

==> figs/latex/macros/rules.tex <==

%\newcommand{\AccSym}{\uparrow}
% \newcommand{\AccSym}{\tick}
%%\RequirePackage{pifont}
%% \newcommand{\tick}{\ding{51}}
%% \newcommand{\AccSym}{\tick}

\RequirePackage{amssymb}
\newcommand{\AccSym}{\surd}


%\newcommand{\RejSym}{\downarrow}
\RequirePackage{pifont}
%\newcommand{\RejSym}{\text{\ding{53}}}
\newcommand{\RejSym}{\,\mathsf{x}\,}

% \newcommand{\ACC}[1]{\ensuremath{\overset{#1}{\AccSym}}}
 \newcommand{\ACC}[1]{\ensuremath{{\AccSym}\hspace{-0.7em}{\overset{#1}{\text{\phantom{x}}}}}}
 \newcommand{\ACCa}{\ACC{s}}
 \newcommand{\REJ}[1]{\ensuremath{\overset{#1}{\RejSym}}}
 \newcommand{\REJa}{\REJ{s}}
 \newcommand{\DER}[1]{\ensuremath{\overset{#1}{\Into}}}
 \newcommand{\DERa}{\DER{s}}

 \newcommand{\BasicAcceptRuleA}{\ell \ACCa\;\;\text{(if $s\models \ell$)}}
 \newcommand{\BasicAcceptRuleB}{\ell \REJa\;\;\text{(if $s\nmodels \ell$)}}
 \newcommand{\BasicNextRule}{\ell \DERa \F}


 \newcommand{\ORAcceptRuleA}{
   \AxiomC{$x\ACCa$}
   %\LeftLabel{\ORAcceptRuleALabel}
   \UnaryInfC{$x \OR y \ACCa$}
   \DisplayProof
 }
 \newcommand{\ORAcceptRuleB}{
   \AxiomC{$y\ACCa$}
   %\LeftLabel{\ORAcceptRuleALabel}
   \UnaryInfC{$x \OR y \ACCa$}
   \DisplayProof
 }
 \newcommand{\ORAcceptRuleC}{
      \AxiomC{$x\REJa$}
      \AxiomC{$y\REJa$}
      %\LeftLabel{\ORAcceptRuleALabel}
      \BinaryInfC{$x \OR y \REJa$}
      \DisplayProof
 }
 \newcommand{\OrNextRule}{
      \AxiomC{$x\DERa x'$}
      \AxiomC{$y\DERa y'$}
      %\LeftLabel{\ORAcceptRuleALabel}
      \BinaryInfC{$x \OR y \DERa x' \OR y'$}
      \DisplayProof
 }

 \newcommand{\AndAcceptRuleA}{
   \AxiomC{$x\REJa$}
   %\LeftLabel{\ORAcceptRuleALabel}
   \UnaryInfC{$x \AND y \REJa$}
   \DisplayProof
   
 }
 \newcommand{\AndAcceptRuleB}{
   \AxiomC{$y\REJa$}
   %\LeftLabel{\ORAcceptRuleALabel}
   \UnaryInfC{$x \AND y \REJa$}
   \DisplayProof
}
\newcommand{\AndAcceptRuleC}{
  \AxiomC{$x\ACCa$}
  \AxiomC{$y\ACCa$}
  %\LeftLabel{\ORAcceptRuleALabel}
  \BinaryInfC{$x \AND y \ACCa$}
  \DisplayProof
}
\newcommand{\AndNextRule}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  %\LeftLabel{\ORAcceptRuleALabel}
  \BinaryInfC{$x \AND y \DERa x' \AND y'$}
  \DisplayProof
}

\newcommand{\SeqAcceptRule}{
  x \SEQ y \REJa
}

\newcommand{\SeqNextRuleA}{
  \AxiomC{$x\ACCa$}
  \AxiomC{$x\DERa x'$}
  %\LeftLabel{\ORAcceptRuleALabel}
  \BinaryInfC{$x \SEQ y \DERa x'\SEQ y \OR y$}
  \DisplayProof
}
\newcommand{\SeqNextRuleB}{
  \AxiomC{$x\REJa$}
  \AxiomC{$x\DERa x'$}
  %\LeftLabel{\ORAcceptRuleALabel}
  \BinaryInfC{$x \SEQ y \DERa x'\SEQ y$}
  \DisplayProof
}

\newcommand{\PowAcceptRuleA}{
  \AxiomC{$y\ACCa$}
  \UnaryInfC{$x^z y \ACCa$}
  \DisplayProof
}
\newcommand{\PowAcceptRuleB}{
  \AxiomC{$y\REJa$}
  \UnaryInfC{$x^z y \REJa$}
  \DisplayProof
}
\newcommand{\PowNextRuleA}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  \AxiomC{$z\DERa z'\;\;\;\;z\REJa$}
  \TrinaryInfC{$x^z y \DERa y' \OR (x' \AND (z' \SEQ x^z y))\text{\phantom{$\OR x^z y$}}$}
  \DisplayProof
}
\newcommand{\PowNextRuleB}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  \AxiomC{$z\DERa z'\;\;\;\;z\ACCa$}
  \TrinaryInfC{$x^z y \DERa y' \OR (x' \AND (z' \SEQ x^z y \OR x^z y))$}
  \DisplayProof
}

\newcommand{\DualPowAcceptRuleA}{
  \AxiomC{$y\REJa$}
  \UnaryInfC{$x_z y \REJa$}
  \DisplayProof
}
\newcommand{\DualPowAcceptRuleB}{
  \AxiomC{$y\ACCa$}
  \AxiomC{$x\ACCa$}
  \BinaryInfC{$x_z y \ACCa$}
  \DisplayProof
}
\newcommand{\DualPowAcceptRuleC}{
  \AxiomC{$y\ACCa$}
  \AxiomC{$x\REJa$}
  \BinaryInfC{$x_z y \REJa$}
  \DisplayProof
}



\newcommand{\DualPowNextRuleA}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  \AxiomC{$z\DERa z'\;\;\;\;z\REJa$}
  \TrinaryInfC{$x_z y \DERa y' \AND (x' \OR (z' \SEQ x_z y))\text{\phantom{$\OR x^z y$}}$}
  \DisplayProof
}
\newcommand{\DualPowNextRuleB}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  \AxiomC{$z\DERa z'\;\;\;\;z\ACCa$}
  \TrinaryInfC{$x_z y \DERa y' \AND (x' \OR (z' \SEQ x_z y \OR x_z y))$}
  \DisplayProof
}

\newcommand{\EquationAcceptRuleA}{
  \AxiomC{$\phi(x_1,\ldots) \ACCa$}
  \UnaryInfC{$\phi(x_1,\ldots) \ACCa_\Eqs$}
  \DisplayProof 
}

\newcommand{\EquationAcceptRuleB}{
  \AxiomC{$\phi(x_1,\ldots) \REJa$}
  \UnaryInfC{$\phi(x_1,\ldots) \REJa_\Eqs$}
  \DisplayProof 
}

\newcommand{\EquationNextRule}{ 
  \AxiomC{$\phi(x_1,\ldots,x_n) \DERa \phi'(x_1,\ldots,x_n)$} 
  \UnaryInfC{$\phi \DERa_\Eqs
    \phi'(\phi_{x_1},\ldots,\phi_{x_n})$} 
  \DisplayProof 
}


==> figs/latex/programs.tex <==
\newcommand{\RefFigListClass}{\ref{fig:programs}(a)\xspace}
\newcommand{\RefFigMGC}      {\ref{fig:programs}(b)\xspace}
\newcommand{\RefFigSearch}   {\ref{fig:programs}(c)\xspace}
\newcommand{\RefFigLocate}   {\ref{fig:programs}(d)\xspace}
\newcommand{\RefFigAdd}      {\ref{fig:programs}(e)\xspace}
\newcommand{\RefFigRemove}   {\ref{fig:programs}(f)\xspace}

\newcommand{\RefFigListClassGhost}{\ref{fig:programs:ghost}(a)\xspace}
\newcommand{\RefFigLocateGhost}		{\ref{fig:programs:ghost}(b)\xspace}
\newcommand{\RefFigAddGhost}			{\ref{fig:programs:ghost}(c)\xspace}
\newcommand{\RefFigRemoveGhost}		{\ref{fig:programs:ghost}(d)\xspace}

\newcommand{\FigLabel}[1]{\multicolumn{1}{c}{#1}}
\newcommand{\FigLabelWide}[1]{\multicolumn{3}{c}{#1}}

%
% Figures for data structure
%

\begin{SaveVerbatim}{list-data}
class List {
     Node list;
}
\end{SaveVerbatim}

\begin{SaveVerbatim}{list-data-space}
class List {
     Node list;

}
\end{SaveVerbatim}


\begin{SaveVerbatim}{node-data}
class Node {
     Value val;
     Node next;
     Lock lock;
}
\end{SaveVerbatim}

\newcommand{\DataStructuresBody}{
  \begin{tabular}{l}
    \renewcommand{\arraystretch}{0.4}
    $\begin{array}{l}
      \class \: \List \: \{ \\
      \mhs \Node \: \tList ;\\
      \}
    \end{array}$ \\ \\ \\
    \renewcommand{\arraystretch}{0.4}
    $\begin{array}{l}
      \class \: \Node \: \{ \\
      \mhs \Value \: \val ;\\
      \mhs \Node \: \tNext ;\\
      \mhs \Lock \: \lock ;\\
      \}
    \end{array}$
  \end{tabular}
}
\newcommand{\DataStructuresFig}{
\begin{minipage}[c]{3.7cm}
  \DataStructuresBody
\label{fig:listclass}
\end{minipage}
}

%
% Figures for most generate cliente "decide"
%
\newcommand{\MGCBody}{
  \begin{algorithmic}[1]
    \While {$\true$}
    \State $e := \NondetChooseElem$
    \State $\Nondet$
    \State $\left[ \begin{array}{l}
	\Call \search(e) \\
	\ProgOr \\
	\Call \add(e) \\
	\ProgOr \\
	\Call \remove(e)
      \end{array} \right]$
    \EndWhile
  \end{algorithmic}
}

\begin{SaveVerbatim}[fontfamily=courier]{mgc-prg}
0:  while true
1:     e:= NonDet();
2:     select
3:        search(e);
4:     or
5:        add(e);
6:     or
7:        remove(e);
8:  end;
\end{SaveVerbatim}

\newcommand{\MGCPrg}{
  \begin{minipage}[c]{5.0cm}
    \MGCBody
  \end{minipage}
}
\newcommand{\MGCFig}{
  \begin{minipage}[c]{4.1cm}
    \MGCBody
    \label{fig:mgc}
  \end{minipage}
}

%
% Figure for "search" 
%
\begin{SaveVerbatim}{search-prog}
20:  prev, cur := locate (e);
21:  if curr.val = e then
22:      result := true;
23:  else
24:      result := false;
25:  curr.unlock();
26:  prev.unlock();
27:  return result;
\end{SaveVerbatim}

\newcommand{\SearchBody}{
  \begin{algorithmic}[1]
    \State $\prev, \curr := \locate(e)$
    \If {$\curr.\val = e$}
    \State $\result := \true$
    \Else
    \State $\result := \false$
    \EndIf
    \State $\curr.\unlock()$
    \State $\prev.\unlock()$
    \State \tbf{return} $\result$
  \end{algorithmic}
}
\newcommand{\SearchPrg}{
  \begin{minipage}[c]{3.9cm}
    \SearchBody
  \end{minipage}
}
\newcommand{\SearchFig}{
\begin{minipage}[c]{3.9cm}
  \SearchBody
\label{fig:search}
\end{minipage}
}

%
% Figure for "locate"
%
\begin{SaveVerbatim}{locate-prog}
 9:  prev := Head;
10:  prev.lock();
11:  curr := prev.next;
12:  curr.lock();
13:  while curr.val < e do
14:      prev.unlock();
15:      prev := curr;
16:      curr := curr.next;
17:      curr.lock();
18:  end;
19:  return (prev,curr)
\end{SaveVerbatim}

\newcommand{\LocateBody}{
\begin{algorithmic}[1]
\State $\prev := \Head$
\State $\prev.\lock()$
\State $\curr := \prev.\tNext$
\State $\curr.lock()$
\While {$\curr.\val < e$}
	\State $\prev.\unlock()$
	\State $\prev := \curr$
	\State $\curr := \curr.\tNext$
	\State $\curr.\lock()$
\EndWhile
\State \tbf{return} $(\prev, \curr)$
\Statex
\end{algorithmic}
}

\newcommand{\LocatePrg}{
  \begin{minipage}[c]{3.7cm}
    \LocateBody
  \end{minipage}
}

\newcommand{\LocateFig}{
\begin{minipage}[c]{3.7cm}
  \LocateBody
\label{fig:locate}
\end{minipage}
}

%
% Figure for "add"
%
\begin{SaveVerbatim}{add-prog}
28:  prev, curr := locate(e);
29:  if curr.val != e then
30:      aux := new Node(e);
31:      aux.next := curr;
32:      prev.next := aux;
33:      result := true;
34:  else
35:      result := false;
36:  end;
37:  prev.unlock();
38:  curr.unlock();
39:  return result;
\end{SaveVerbatim}



\newcommand{\AddBody}{
\begin{algorithmic}[1]
\State $\prev, \curr := \locate(e)$
\If {$\curr.\val \neq e$}
	\State $\aux := \New \Node(e)$
	\State $\aux.\tNext := \curr$
	\State $\prev.\tNext := \aux$
	\State $\result := \true$
\Else
	\State $\result := \false$
\EndIf
\State $\prev.\unlock()$
\State $\curr.\unlock()$
\State \tbf{return} $\result$
\end{algorithmic}
}

\newcommand{\AddPrg}{
  \begin{minipage}[c]{4.1cm}
    \AddBody
  \end{minipage}
}

\newcommand{\AddFig}{
\begin{minipage}[c]{4.1cm}
  \AddBody
  \label{fig:add}
\end{minipage}
}

%
% Figure for "remove"
%
\begin{SaveVerbatim}{remove-prog}
40:  prev, curr := locate(e);
41:  if curr.val == e then
42:      aux := curr.next;
43:      prev.next := aux;
44:      result := true;
45:  else
46:      result := false;
47:  end;
48:  prev.unlock();
49:  curr.unlock();
50:  return result;
\end{SaveVerbatim}


\newcommand{\RemoveBody}{
    \begin{algorithmic}[1]
      \State $\prev, \curr := \locate(e)$
      \If {$\curr.\val = e$}
      \State $\aux := \curr.\tNext$
      \State $\prev.\tNext := \aux$
      \State $\result := \true$
      \Else
      \State $\result := \false$
      \EndIf
      \State $\prev.\unlock()$
      \State $\curr.\unlock()$
      \State \tbf{return} $\result$
      \Statex
    \end{algorithmic}
}

\newcommand{\RemovePrg}{
  \begin{minipage}[c]{3.9cm}
    \RemoveBody
  \end{minipage}
}


\newcommand{\RemoveFig}{
  \begin{minipage}[c]{3.9cm}
    \RemoveBody
    \label{fig:remove}
  \end{minipage}
}




%
% Figures for data structure
%
\newcommand{\DataStructuresGhostBody}{
	\begin{tabular}{cc}
		\renewcommand{\arraystretch}{0.4}
		$\begin{array}{l}
			\class \: \List \: \{ \\
			\mhs \Node \: \tList ;\\
			\hs{0.2} \fbox{ \begin{array}{l}
				\rgn \: r; \\
			\end{array}}\\
		\}
		\end{array}$ & \hs{2} $\begin{array}{l}
			\class \: \Node \: \{ \\
			\mhs \Value \: \val ;\\
			\mhs \Node \: \tNext ;\\
			\mhs \Lock \: \lock ;\\
		\}
	\end{array}$
	\end{tabular}
}

\newcommand{\DataStructuresGhostFig}{
\begin{minipage}[c]{6.5cm}
	\DataStructuresGhostBody
\label{fig:conclists:ghost}
\end{minipage}
}


%
% Figure for "locate" extended with ghost fields
%

\newcommand{\LocateGhostBody}{
	\begin{algorithmic}[1]
		\State $\prev := \Head$
		\State $\prev.\lock()$
		\State $\curr := \prev.\tNext$
		\State $\curr.lock()$
		\While {$\curr.\val < e$}
			\State $\prev.\unlock()$
			\State $\prev := \curr$
			\State $\curr := \curr.\tNext$
			\State $\curr.\lock()$
		\EndWhile
		\State \tbf{return} $(\prev, \curr)$
		\vspace{0.8cm}
	\end{algorithmic}
}


\newcommand{\LocateGhostFig}{
\begin{minipage}[c]{4.2cm}
	\LocateGhostBody
\label{fig:locate:ghost}
\end{minipage}
}


%
% Figure for "add" extended with ghost fields
%
\newcommand{\AddGhostBody}{
	\begin{algorithmic}[1]
		\State $\prev, \curr := \locate(e)$
		\If {$\curr.\val \neq e$}
			\State $\aux := \New \Node(e)$
			\State $\aux.\tNext := \curr$
			\State $\prev.\tNext := \aux$
			\Statex $\hs{0.7}\fbox{
				\begin{array}{l}
					l.r := l.r \cup \sreg{\aux} \\
				\end{array}}$
			\State $\result := \true$
		\Else
			\State $\result := \false$
		\EndIf
		\State $\prev.\unlock()$
		\State $\curr.\unlock()$
		\State \tbf{return} $\result$
	\end{algorithmic}
}


\newcommand{\AddGhostFig}{
\begin{minipage}[c]{4.2cm}
	\AddGhostBody
	\label{fig:add:ghost}
\end{minipage}
}


%
% Figure for "remove" extended with ghost fields
%
\newcommand{\RemoveGhostBody}{
		\begin{algorithmic}[1]
			\State $\prev, \curr := \locate(e)$
			\If {$\curr.\val = e$}
				\State $\aux := \curr.\tNext$
				\State $\prev.\tNext := \aux$
				\Statex $\hs{0.7}\fbox{
					\begin{array}{l}
						l.r := l.r - \sreg{\curr} \\
					\end{array}}$
				\State $\result := \true$
			\Else
				\State $\result := \false$
			\EndIf
			\State $\prev.\unlock()$
			\State $\curr.\unlock()$
			\State \tbf{return} $\result$
			\Statex
		\end{algorithmic}
}


\newcommand{\RemoveGhostFig}{
	\begin{minipage}[c]{4.3cm}
		\RemoveGhostBody
		\label{fig:remove:ghost}
  \end{minipage}
}



\begin{SaveVerbatim}{skiplist-data}
class Skiplist {
	Node* head;
	Node* tail;
	int maxLevel;

}
\end{SaveVerbatim}

\begin{SaveVerbatim}{skiplist-node-data}
class Node {
	Value v;
	Key k;
	Array<Node*>(4) next;
}
\end{SaveVerbatim}



==> figs/latex/theories.tex <==
%
% T_{fSeq} to T_{path} Auxiliary Functions
%
\newcommand{\TPathFig}{
\renewcommand{\arraystretch}{1}
\centering
\begin{tabular}{|c|}
\hline
$\fApp : \sSeq \times \sSeq \to \sSeq$ \\
\hline
$\fApp (\fNil, l) = l$ \\
$\fApp(\fCons(a,l), l') = \fCons(a, \fApp(l, l'))$ \\
\hline
\hline
$\fSeqToSet : \sSeq \to \sSet$ \\
\hline
$\fSeqToSet (\fNil) = \emptyset$ \\
$\fSeqToSet (\fCons(a,l)) = \{ a \} \cup \fSeqToSet(l)$ \\
\hline
\hline
$\fIsPath : \sSeq$ \\
\hline
$\fIsPath(\fNil)$ \\
$\fIsPath(\fCons(a, \fNil))$ \\
$\{a\} \nsubseteq \fSeqToSet(l) \land \fIsPath(l) \Impl
	\fIsPath(\fCons(a,l))$ \\
\hline
\hline
$\fLast : \sSeq \to \sAddr$ \\
\hline
$\fLast(\fCons(a, \fNil)) = a$ \\
$l \neq \fNil \Impl \fLast(\fCons(a, l)) = \fLast(l)$ \\
\hline
\hline
$\pIsReachK : \sMem \times \sAddr \times \sAddr \times \sLevelK$ \\
\hline
$\pIsReachK(m, a, a, l)$ \\
$m[a].\fNext[l] = a' \land \pIsReach(m, a', b, l)
	\Impl \pIsReach(m, a, b, l)$ \\
\hline
\hline
$\pIsReachKP : \sMem \times \sAddr \times \sAddr \times \sLevelK
	\times \sSeq$ \\
\hline
$\pIsReachKP(m, a, a, l, \fNil)$ \\
$m[a].\fNext[l] = a' \land \pIsReachP(m, a', b, l, p) \Impl
	\pIsReachP(m, a, b, l, \fCons(a, p))$ \\
\hline
\hline
$\fFirstMarked : \sMem \times \sSeq \times \sLevelK \times \sAddr$ \\
\hline
$\fFirstMarked (m, \fNil, l, \fNull)$ \\
$p \neq \fNil \land p = \fCons(j, q) \land m[j].\fLockID[l] \neq \oslash
	\Impl \fFirstMarked(m, p, l, j)$ \\
$p \neq \fNil \land p = \fCons(j, q) \land m[j].\fLockID[l] = \oslash
	\land \fFirstMarked(m, q, l, i)
		\Impl \fFirstMarked(m, p, l, i)$ \\
\hline
\hline
$\pOrdPath : \sMem \times \sSeq$ \\
\hline
$\pOrdPath(h, \fNil)$ \\
$h[a].\fNext[\fLevel{0}] = a' \land h[a].\fKey \pOrd h[a'].\fKey \land
	p = \fCons(a, q) \land \pOrdPath(h, q) \Impl \pOrdPath(h, p)$ \\
\hline
\end{tabular}
}


%
% TLLpL Auxiliary Functions
%
\newcommand{\AuxiliaryFunctions}{
\centering
\begin{tabular}{|c|}
\hline
$\List : \sMem \times \sAddr \times \sSet$ \\
\hline
$\begin{array}{lcl}
	\List(h,a,r) & \Iff & \fNull \in \fAddrToSet(h, a)
		\land r = \fPathToSet(\fGetp(h, a, \fNull)) \\
\end{array}$\\
\hline
\hline
$\fa : \sMem \times \sAddr \to \sPath$ \\
\hline
$\fa(h,n) = \begin{cases}
		\fEpsilon & \trm{if } n = \fNull \\
		\fGetp(h, h[n].\fNext, \fNull) & \trm{if } n \neq \fNull \\
		\end{cases}$ \\
\hline
%
% Begin: Function removed to reduce space
%
%\hline
%$\fb : \sMem \times \sAddr \times \sAddr \times \sPath$ \\
%\hline
%$\begin{array}{lcl}
%\fb(h, n, m, p) & \Iff & (n = \fNull \land p = \fEpsilon)
%	\lor \; \big(n \neq \fNull \land \pReach(h,n,m,\tilde{p})\\
%		&& \hs{3.5} \land \; m = \fNull
%			\Impl \pAppend(p, \fNull, \tilde{p}) \\
%		&& \hs{3.5} \land \; m \neq \fNull
%			\Impl \pAppend(p, [m], \tilde{p}) \big) \\
%\end{array}$ \\
%\hline
\hline
$\LastMarked : \sMem \times \sPath \to \sAddr$ \\
\hline
$\LastMarked(m, p) = \fFirstLocked(m, \fRev(p))$ \\
\hline
\hline
$\NoMarks : \sMem \times \sPath$ \\
\hline
$\NoMarks(m,p) \Iff \fFirstLocked(m,p) = \fNull$ \\
\hline
\hline
$\SomeMark : \sMem \times \sPath$ \\
\hline
$\SomeMark(m,p) \Iff \fFirstLocked(m,p) \neq \fNull$ \\
\hline
\end{tabular}
}



%
% TSLK Signature
%
\newcommand{\TSLKSignature}{
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Signature & \hs{0.1} Sorts \hs{0.1} & Functions & Predicates \\
\hline
\hline
\sigLevelK &
	$\begin{array}{c}
		\sLevelK
	\end{array}$ &
	$\begin{array}{lcl}
		0,1, \ldots, \K-1 & : & \sLevelK \\
	\end{array}$ &
	$\begin{array}{lcl}
		< : \sLevelK \times \sLevelK
	\end{array}$\\
\hline
\sigOrd &
	$\begin{array}{c}
		\sOrd
	\end{array}$ &
	$\begin{array}{lcl}
		\fZero & : & \sOrd \\
		\fInfty & : & \sOrd \\
	\end{array}$ &
	$\begin{array}{lcl}
		\pOrd & : & \sOrd \times \sOrd \\
	\end{array}$ \\
\hline
\sigThId &
	$\begin{array}{c}
		\sThId
	\end{array}$ &
	$\begin{array}{lcl}
		\oslash & : & \sThId \\
	\end{array}$ & \\
\hline
\hline
\sigCells &
	$\begin{array}{c}
		\sCell \\ \sElem \\ \sOrd \\ \sAddr \\ \sThId
	\end{array}$ &
	$\begin{array}{lcl}
		\fError & : & \sCell \\
		\fMkcell & : & \sElem \times \sOrd \times \sAddr^{\K}
			\times \sThId^{\K} \to \sCell \\
		\_.\fData & : & \sCell \to \sElem \\
		\_.\fKey & : & \sCell \to \sOrd \\
		\_.\fNext \lbrack \_ \rbrack & : & \sCell \times \sLevelK
			\to \sAddr \\
		\_.\fLockID \lbrack \_ \rbrack & : & \sCell
			\times \sLevelK \to \sThId \\
		\_.\fLock \lbrack \_ \rbrack & : & \sCell \times \sLevelK	
			\to \sThId \to \sCell \\
		\_.\fUnlock \lbrack \_ \rbrack & : & \sCell
			\times \sLevelK \to \sCell \\
	\end{array}$ & \\
\hline
\sigMemory &
	$\begin{array}{c}
		\sMem \\ \sAddr \\ \sCell
	\end{array}$ &
	$\begin{array}{lcl}
		\fNull & : & \sAddr \\
		\_[\_] & : & \sMem \times \sAddr \to \sCell \\
		\fUpd & : & \sMem \times \sAddr \times \sCell \to \sMem
	\end{array}$ & \\
\hline
\sigReach &
	$\begin{array}{c}
		\sMem \\ \sAddr \\ \sPath
	\end{array}$ &
	$\begin{array}{lcl}
		\fEpsilon & : & \sPath \\
		\lbrack \_ \rbrack & : & \sAddr \to \sPath
	\end{array}$ &
	$\begin{array}{lcl}
		\pAppend & : & \sPath \times \sPath \times \sPath \\
		\pReachK & : & \sMem \times \sAddr \times \sAddr \\
				&& \mhs \times \; \sLevelK \times \sPath \\
	\end{array}$ \\
\hline
\hline
\sigSets &
	$\begin{array}{c}
		\sAddr \\ \sSet
	\end{array}$ &
	$\begin{array}{lcl}
		\emptyset & : & \sSet \\
		\{ \_ \} & : & \sAddr \to \sSet \\
		\cup, \cap, \setminus & : & \sSet \times \sSet \to \sSet
	\end{array}$ &
	$\begin{array}{lcl}
		\in & : & \sAddr \times \sSet \\
		\subseteq & : & \sSet \times \sSet
	\end{array}$ \\
\hline
\sigSetsT &
	$\begin{array}{c}
		\sThId \\ \sSetT
	\end{array}$ &
	$\begin{array}{lcl}
		\stEmpty & : & \sSetT \\
		\stSingle{\_} & : & \sThId \to \sSetT \\
		\stCup, \stCap, \stSubst & : & \sSetT \times \sSetT \to \sSetT
	\end{array}$ &
	$\begin{array}{lcl}
		\stIn & : & \sThId \times \sSetT \\
		\stSubset & : & \sSetT \times \sSetT
	\end{array}$ \\
\hline
\sigMrgn &
	$\begin{array}{c}
		\sMrgn, \\ \sAddr \\ \sLevelK
	\end{array}$ &
	$\begin{array}{lcl}
		\mrgnEmpty & : & \sMrgn \\
		\mrgnSingle{\_, \_} & : & \sAddr \times \sLevelK \to \sMrgn \\
		\mrgnCup, \mrgnCap, \mrgnMinus & : & \sMrgn \times \sMrgn
			\to \sMrgn
	\end{array}$ &
	$\begin{array}{lcl}
		\mrgnIn & : & \sAddr \times \sLevelK \times \sMrgn \\
		\mrgnSubset & : & \sMrgn \times \sMrgn \\
		\mrgnDisj & : & \sMrgn \times \sMrgn
	\end{array}$ \\
\hline
\hline
\sigBridge &
	$\begin{array}{c}
		\sMem \\ \sAddr \\ \sSet \\ \sPath
	\end{array}$ &
	$\begin{array}{lcl}
		\fPathToSet & : & \sPath \to \sSet \\
		\fAddrToSetK & : & \sMem \times \sAddr \times \sLevelK
			\to \sSet \\
		\fGetpK & : & \sMem \times \sAddr \times \sAddr \times
			\sLevelK \to \sPath \\
		\fFirstLockedK & : & \sMem \times \sPath \times \sLevelK
			\to \sAddr
	\end{array}$ &
	$\begin{array}{lcl}
		\pOrdList & : & \sMem \times \sPath \\
	\end{array}$ \\
\hline
\end{tabular}
}


%
% TSLK Interpretations
%
\newcommand{\TSLKInterpretationsOne}{
\centering
\begin{tabular}{|c|p{10.5cm}|}
\hline
\multicolumn{2}{|c|}{Interpretation of sort symbols: \sAddr, \sElem, 
\sThId, \sLevelK, \sOrd, \sCell, \sMem, \sPath, \sSet, \sSetT and \sMrgn}
\\
\hline
\hline
\multicolumn{2}{|l|}{
Each sort $\sigma$ in \sigTSLK is mapped to a non-empty set $\Ais{\sigma}$ 
such that:} \\
\multicolumn{2}{|l|}{
\begin{tabular}{clcl}
	(a) &$\Ais{\sAddr}$ and $\Ais{\sElem}$ are discrete sets &
	(b) &$\Ais{\sThId}$ is a discrete set containing symbol $\oslash$ \\
	(c) &$\Ais{\sLevelK}$ is the finite collection 0,\ldots,\K-1 &
	(d) &$\Ais{\sOrd}$ is a collection of total ordered identifiers \\
	(e) &$\Ais{\sCell} = \Ais{\sElem} \times \Ais{\sOrd} \times 
		\Ais{\sAddr}^{\K} \times \Ais{\sThId}^{\K}$ &
	(f) &$\Ais{\sMem} = \Ais{\sCell}^{\Ais{\sAddr}}$ \\
	(g) &$\Ais{\sPath}$ is the set of all finite sequences of &
	(h) &$\Ais{\sSet}$ is the power-set of $\Ais{\sAddr}$ \\
		& \hs{0.5} (pairwise) distinct elements of $\Ais{\sAddr}$ &
	(i) &$\Ais{\sSetT}$ is the power-set of $\Ais{\sThId}$ \\
	(j) &$\Ais{\sMrgn}$ is the power-set of
		$\Ais{\sAddr} \times \Ais{\sLevelK}$ &
\end{tabular}
} \\
\hline
\hline
Signature & Interpretation \\
\hline
%\hline
%\sigLevelK &
%	\begin{tabular}{p{9.7cm}}
%		$\inter{\fLevel{i}}{\Ai} \neq \inter{\fLevel{j}}{\Ai}$
%			when $i \neq j$
%	\end{tabular} \\
\hline
\sigOrd &
	\begin{tabular}{p{9.7cm}}
		$x \inter{\pOrd}{\Ai} y \land y \inter{\pOrd}{\Ai} x
			\Impl x = y$ for any $x, y \in \Ais{\sOrd}$ \\
		$x \inter{\pOrd}{\Ai} y \land y \inter{\pOrd}{\Ai} z
			\Impl x \inter{\pOrd}{\Ai} z$
			for any $x, y, z \in \Ais{\sOrd}$ \\
		$x \inter{\pOrd}{\Ai} y \lor y \inter{\pOrd}{\Ai} x$
			for any $x, y \in \Ais{\sOrd}$ \\
		$\inter{\fZero}{\Ai} \inter{\pOrd}{\Ai} x \land
		x \inter{\pOrd}{\Ai} \inter{\fInfty}{\Ai}$
			for any $x \in \Ais{\sOrd}$ \\
%		$x \neq \inter{\fInfty}{\Ai} \Impl
%			x \inter{\pOrd}{\Ai} \inter{\fSucc}{\Ai}(x)$
%			for any $x \in \Ais{\sOrd}$ \\
	\end{tabular} \\
\hline
\hline
\sigCells &
	\begin{tabular}{p{11.5cm}}
		\begin{compactitem}
		\item $\inter{\fMkcell}{\Ai} (e, k, a_0, \ldots, a_{\K-1},
						t_0, \ldots, t_{\K-1}) =
			\langle e, k, a_0, \ldots, a_{\K-1},
				t_0, \ldots, t_{\K-1} \rangle$
			for each
			$e \in \Ais{\sElem}$, $i \in \Ais{\sOrd}$,
			$a_0, \ldots, a_{\K-1} \in \Ais{\sAddr}$
			and $t_0, \ldots, t_{\K-1} \in \Ais{\sThId}$
		\item $\langle e, k, \vect{a}, \vect{t} \rangle
				.\inter{\fData}{\Ai} = e$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$
			and $\vect{t} \in \Ais{\sThId}^{\K}$
		\item $\langle e, k, \vect{a}, \vect{t} \rangle
				.\inter{\fKey}{\Ai} = k$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$
			and $\vect{t} \in \Ais{\sThId}^{\K}$
		\item $\langle e, k, a_0, \ldots, a_{\K-1}, \vect{t} \rangle
				.\inter{\fNext}{\Ai}[j] = a_j$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$a_0 \ldots, a_{\K-1} \in \Ais{\sAddr}$,
			$j \in \Ais{\sLevelK}$
			and $\vect{t} \in \Ais{\sThId}^{\K}$ and
		\item $\langle e, k, \vect{a}, t_0, \ldots, t_{\K-1} \rangle
				.\inter{\fLockID}{\Ai}[j] = t_{j}$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$,
			$j \in \Ais{\sLevelK}$
			and $t_0, \dots, t_{\K-1} \in \Ais{\sThId}$
		\item $\langle e, k, \vect{a}, t_0, \ldots, t_{\K-1} \rangle
				.\inter{\fLock}{\Ai}[j](t') =
			\langle e, k, \vect{a},
				t_0, \ldots, t_{j-1}, t',
				t_{j+1}, \ldots, t_{\K-1}
			\rangle$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$,
			$j \in \Ais{\sLevelK}$
			and $t_0, \ldots, t_{\K-1}, t' \in \Ais{\sThId}$
		\item $\langle e, k, \vect{a}, t_0, \ldots, t_{\K-1} \rangle
				.\inter{\fUnlock}{\Ai}[j] =
			\langle e, k, \vect{a},
				t_0, \ldots, t_{j-1}, \oslash,
				t_{j+1}, \ldots, t_{\K-1}
			\rangle$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$,
			$j \in \Ais{\sLevelK}$
			and $t_0, \ldots, t_{\K-1} \in \Ais{\sThId}$
		\item $\inter{\fError}{\Ai}.\inter{\fNext}{\Ai} =
			\inter{\fNull}{\Ai}$
		\end{compactitem}
	\end{tabular} \\
\hline
\sigMemory &
	\begin{tabular}{p{9.7cm}}
		\begin{compactitem}
		\item $m\inter{[a]}{\Ai} = m(a)$ for each $m \in \Ais{\sMem}$
			and $a \in \Ais{\sAddr}$
		\item $\inter{\fUpd}{\Ai}(m,a,c) = m_{a \mapsto c}$ for each
			$m \in \Ais{\sMem}$, $a \in \Ais{\sAddr}$ and
			$c \in \Ais{\sCell}$
		\item $\inter{m}{\Ai}(\inter{\fNull}{\Ai}) = 
			\inter{\fError}{\Ai}$
			for each $m \in \Ais{\sMem}$
		\end{compactitem}
	\end{tabular} \\
\hline
\sigReach &
	\begin{tabular}{p{11cm}}
		\begin{compactitem}
		\item $\inter{\fEpsilon}{\Ai}$ is the empty sequence
		\item $\inter{[i]}{\Ai}$ is the sequence containing $i \in 
			\Ais{\sAddr}$ as the only element
		\item $\left(\left[i_1,\ldots, i_n\right], \left[j_1, \ldots, 
			j_m\right], \left[i_1,\ldots, i_n, j_1,
				\ldots, j_m\right]
			\right) \in \inter{\pAppend}{\Ai}$ iff $i_k$
		and $j_l$ are all distinct
		\item $(m, \aInit, \aEnd, l, p) \in \inter{\pReachK}{\Ai}$
			iff $\aInit=\aEnd$ and $p = \fEpsilon$, or
		there exist addresses $a_1, \ldots, a_n \in \Ais{\sAddr}$ such 
		that:
		\end{compactitem} \\
		\hs{1.5} $\begin{array}{ll}
			\trm{(a) } p = [a_1, \ldots, a_n]  \phantom{aaaa}&
			\trm{(c) } m(a_r).\inter{\fNext}{\Ai}[l]
				= a_{r+1}, \trm{for } 1 \leq r < n \\
			\trm{(b) } a_1 = \aInit &
			\trm{(d) } m(a_n).\inter{\fNext}{\Ai}[l]
				= \aEnd
		\end{array}$
	\end{tabular} \\
\hline
\hline
\sigSets &
	\begin{tabular}{p{11cm}}
		The symbols $\emptyset$, $\{ \_ \}$, $\cup$, $\cap$, 
		$\setminus$, $\in$ and $\subseteq$ are interpreted 
according to
		their standard interpretation over sets of addresses.
	\end{tabular} \\
\hline
\sigSetsT &
	\begin{tabular}{p{11cm}}
		The symbols $\stEmpty$, $\stSingle{\_}$, $\stCup$, $\stCap$, 
		$\stSubst$, $\stIn$ and $\stSubset$ are interpreted according
		to their standard interpretation over sets of thread
		identifiers.
	\end{tabular} \\
\hline
\end{tabular}
}


\newcommand{\TSLKInterpretationsTwo}{
\centering
\begin{tabular}{|c|p{11.7cm}|}
\hline
Signature & Interpretation \\
\hline
\hline
\sigMrgn &
	\begin{tabular}{p{11cm}}
		\begin{compactitem}
		\item $\mrgnEmptyI{\Ai} = \emptyset$
		\item $\mrgnSingleI{a,j}{\Ai} = \{ (a,j) \}$
			for each $a \in \Ais{\sAddr}$
			and $j \in \Ais{\sLevelK}$
		\item $m_1 \mrgnCupI{\Ai} m_2 = m_1 \cup m_2$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\item $m_1 \mrgnCapI{\Ai} m_2 = m_1 \cap m_2$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\item $m_1 \mrgnMinusI{\Ai} m_2 = m_1 \setminus m_2$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\item $m_1 \mrgnSubsetI{\Ai} m_2 \Iff m_1 \subseteq m_2$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\item $(a,j) \mrgnInI{\Ai} m \Iff (a,j) \in m$
			for each $a \in \Ais{\sAddr}$,
			$j \in \Ais{\sLevelK}$ and $m \in \Ais{\sMrgn}$
		\item $m_1 \mrgnDisjI{\Ai} m_2 \Iff m_1 \mrgnCapI{\Ai} m_2
			= \mrgnEmptyI{\Ai}$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\end{compactitem}
	\end{tabular} \\
\hline
\hline
\sigBridge &
	\begin{tabular}{p{11cm}}
		\begin{compactitem}
		\item $\inter{\fPathToSet}{\Ai}(p) = \{ a_1, \ldots, 
			a_n\}$ for $p = [a_1, \ldots, a_n] \in
			\Ais{\sPath}$
		\item $\inter{\fAddrToSetK}{\Ai}(m, a, l) = \big\{
			a' \in \Ais{\sAddr} \:|\: \exists p \in 
			\Ais{\sPath}$ s.t. $(m,a,a',l,p) \in \pReachK
			\big\}$
		\item $\inter{\fGetpK}{\Ai}(m,\aInit,\aEnd,l) =
			\begin{cases}
				p & \text{if } (m,\aInit,\aEnd,l,p)
					\in \inter{\pReachK}{\Ai} \\
				\fEpsilon & \text{otherwise}
			\end{cases}$
		\end{compactitem} \\
			\hspace{1cm} for each $m \in \Ais{\sMem}$,
			$p \in \Ais{\sPath}$, $l \in \Ais{\sLevelK}$
			and $\aInit, \aEnd \in \Ais{\sAddr}$
		\begin{compactitem}
		\item $\inter{\fFirstLocked}{\Ai}\left(m,[a_1, \ldots,
			a_n], l \right) =\left\{
			\begin{array}{ll}
			a_k &
			\trm{if there is } 1 \leq k \leq n \trm{ such that } \\
			& \trm{for all } 1 \leq j < k,
				m[a_j].\fLockID[l] = \oslash \\
			& \trm{and } m[a_k].\fLockID[l] \neq \oslash \\
			\fNull & \trm{otherwise }
			\end{array}
			\right.$
		\item $\inter{\pOrdList}{\Ai}\left(m,p \right)$
			iff $p=\fEpsilon$ or $p = \lbrack a \rbrack$ or
			$p = [a_1, \ldots, a_n]$ with $n \geq 2$ and
			$m(a_i).\inter{\key}{\Ai} \pOrd
				m(a_{i+1}).\inter{\key}{\Ai}$
			for all $1 \leq i < n$,
			for any $m \in \Ais{\sMem}$
		\end{compactitem}
	\end{tabular} \\
\hline
\end{tabular}
}


==> figs/latex/vpl-macros.tex <==
\newcommand{\val}[1]{\ensuremath{[\![ #1 ]\!]}}
\newcommand{\der}[1]{\ensuremath{{\mathop{{ %
            \longrightarrow}}\limits^{{#1}}}\!}} %
\newcommand \tpl[1]{\langle #1 \rangle}
%\newcommand{\RE}{\textsf{RE}\xspace}
\newcommand{\NVPA}{\textsf{NVPA}\xspace}
\newcommand{\VPA}{\textsf{VPA}\xspace}
\newcommand{\NFA}{\textsf{NFA}\xspace}
\newcommand{\VPL}{\textsf{VPL}\xspace}
\newcommand{\CARET}{\textsf{CaRet}\xspace}
\newcommand{\VPLs}{\textsf{VPL}s\xspace}
\newcommand{\VRL}{\textsf{VRL}\xspace}
\newcommand{\VRE}{\textsf{VRE}\xspace}
\newcommand{\EMSO}{\textsf{MSO$_{\mu}$}\xspace}
\newcommand{\MSO}{\textsf{MSO}\xspace}
\newcommand{\XML}{\textsf{XML}\xspace}

\newcommand{\EXPTIME}{{\sffamily EXPTIME}\xspace}

\newcommand{\WM}{\ensuremath{\mathit{WM}}\xspace}
\newcommand{\MR}{\ensuremath{\mathit{MR}}\xspace}
\newcommand{\MC}{\ensuremath{\mathit{MC}}\xspace}
\newcommand{\SWM}{\ensuremath{\mathit{MWM}}\xspace}
\newcommand{\Pu}{\ensuremath{\mathcal{P}}\xspace}
%\newcommand{\Lang}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Au}{\ensuremath{\mathcal{A}}}
\newcommand{\Msubst}{$M$-substitution\xspace}
\newcommand{\Mclosure}{$M$-closure\xspace}
\newcommand{\Sclosure}{$S$-closure\xspace}


\newcommand{\Stilde}{\widetilde{\Sigma}\xspace}
\newcommand{\Scall}{\Sigma_{\mathit{call}}\xspace}
\newcommand{\Sret}{\Sigma_{\mathit{ret}}\xspace}
\newcommand{\Sint}{\Sigma_{\mathit{int}}\xspace}

\newcommand{\SubstOp}[1]{\mathrel{\curvearrowleft_{#1}}}
\newcommand{\SubstBox}{\SubstOp{\Box}}
\newcommand{\MClos}[2]{#1^{\SubstOp{#2}}}
\newcommand{\LangClos}{\MClos{\Lang}{\Box}}
\newcommand{\SClos}[2]{{#1}^{\circlearrowleft_{#2}}}
\newcommand{\SClosure}[1]{\SClos{#1}{\Box}}
\newcommand{\LangSClos}{\SClos{\Lang}{\Box}}



%\newcommand{\DefinedAs}{\,\stackrel{\text{def}}{=}\,}

%\newcommand{\DefOR}{\ensuremath{\;\;\;\big|\;\;\;}}
\newcommand{\DefORmini}{\ensuremath{\;\;\big|\;\;}}

\newcommand{\details}[1]{}

\newcommand{\Outcm}{c\,b\,r}
\newcommand{\UOutcm}{\underline{\Outcm}}

\newcommand{\LSet}{R}
\newcommand{\SSet}{S}

\newcommand{\qin}{\ensuremath{q_{\textit{in}}}}
